Beyond End-to-End VLMs: Leveraging Intermediate Text Representations for Superior Flowchart Understanding

Flowcharts are typically presented as images, driving the trend of using vision-language models (VLMs) for end-to-end flowchart understanding. However, two key challenges arise: (i) Limited controllability--users have minimal influence over the downstream task, as they can only modify input images, while the training of VLMs is often out of reach for most researchers. (ii) Lack of explainability--it is difficult to trace VLM errors to specific causes, such as failures in visual encoding or reasoning. We propose TextFlow, addressing aforementioned issues with two stages: (i) Vision Textualizer--which generates textual representations from flowchart images; and (ii) Textual Reasoner--which performs question-answering based on the text representations. TextFlow offers three key advantages: (i) users can select the type of text representations (e.g., Graphviz, Mermaid, PlantUML), or further convert them into executable graph object to call tools, enhancing performance and controllability; (ii) it improves explainability by helping to attribute errors more clearly to visual or textual processing components; and (iii) it promotes the modularization of the solution, such as allowing advanced LLMs to be used in the Reasoner stage when VLMs underperform in end-to-end fashion. Experiments on the FlowVQA and FlowLearn benchmarks demonstrate TextFlow's state-of-the-art performance as well as its robustness. All code is publicly available.

==> table/extraction_evaluation.tex <==
% \begin{table*}[ht]
% \small
% \centering
% \caption{Performance Comparison of LVLMs on Graphviz, Mermaid, and Plantuml Extraction.}
% \label{tab:extraction_evaluation}
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
% \hline
% \textbf{Model} & \multicolumn{4}{c|}{\textbf{Graphviz}} & \multicolumn{4}{c|}{\textbf{Mermaid}} & \multicolumn{4}{c}{\textbf{Plantuml}} \\
% \hline
% & \multicolumn{2}{c|}{\textbf{Node}} & \multicolumn{2}{c|}{\textbf{Edge}} & \multicolumn{2}{c|}{\textbf{Node}} & \multicolumn{2}{c|}{\textbf{Edge}} & \multicolumn{2}{c|}{\textbf{Node}} & \multicolumn{2}{c}{\textbf{Edge}} \\
% & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 \\
% \hline
% GPT-4o & \textbf{97.21} & \textbf{98.47} & \textbf{88.29} & \textbf{92.87} & \textbf{98.18} & \textbf{99.00} & \textbf{90.26} & \textbf{94.32} &  &  &  &  \\
% Claude-3.5-Sonnet & 87.03 & 91.20 & 54.01 & 62.10 & 94.30 & 96.74 & 83.58 & 89.49 &  &  &  &  \\
% Qwen2-VL-72B & 80.27 & 86.78 & 60.58 & 69.01 & 69.67 & 73.10 & 57.35 & 63.87 &  &  &  &  \\
% Llama3.2-90B & 62.60 & 71.16 & 34.20 & 45.58 & 69.74 & 73.19 & 45.39 & 54.66 &  &  &  &  \\
% Llava-v1.6-110B & 42.40 & 51.18 & 21.38 & 28.97 & 37.09 & 46.84 & 15.13 & 22.57 &  &  &  &  \\
% Qwen2-VL-7B & 36.15 & 39.63 & 18.31 & 23.58 & 28.46 & 37.20 & 8.35 & 11.91 &  &  &  &  \\
% Llama3.2-11B & 40.44 & 49.21 & 12.56 & 18.57 & 10.33 & 12.49 & 4.33 & 5.58 &  &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}


\begin{table*}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\caption{Performance Comparison of LVLMs on Flowchart Extraction, including F1 Score for nodes and edges and Rendering Success Rate. \color{blue} The master students are still working on the annotation and will get the results for those empty entries by today.}
\label{tab:extraction_evaluation}
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\textbf{Model} & \multicolumn{3}{c|}{\textit{Graphviz}} & \multicolumn{3}{c|}{\textit{Mermaid}} & \multicolumn{3}{c}{\textit{PlantUML}} \\
\hline
& Node & Link & Rendering & Node & Link & Rendering & Node & Link & Rendering \\
& F1 & F1 & Success Rate & F1 & F1 & Success Rate & F1 & F1 & Success Rate \\
\hline
GPT-4o & \textbf{0.98} & \textbf{0.93} & \textbf{100} & \textbf{0.99} & \textbf{0.94} & \textbf{100} &  &  &  \\
Claude3.5-Sonnet & 0.95 & 0.87 & \textbf{100} & 0.97 & 0.89 & 98 & 0.98 & 0.91 & 82 \\
Qwen2-VL-72B & 0.92 & 0.78 & \textbf{100} & 0.73 & 0.64 & 74 &  &  &  \\
Llama3.2-90B & 0.71 & 0.46 & 62 & 0.73 & 0.55 & 84 &  &  & 74 \\
Llava-v1.6-110B & 0.51 & 0.29 & 86 & 0.47 & 0.23 & 82 & - & - & 68 \\
Qwen2-VL-7B & 0.47 & 0.28 & 68 & 0.37 & 0.12 & 12 & - & - & 18 \\
Llama3.2-11B & 0.49 & 0.19 & 34 & 0.12 & 0.06 & 8 & - & - & 10 \\
\hline
\end{tabular}
\end{table*}








==> table/ground_truth_replacement.tex <==
\begin{table}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\setlength{\tabcolsep}{5pt} % Adjust column padding
\caption{The table shows the percentage change in accuracy after replacing the representation extracted by GPT-4o with the ground truth.}
\label{tab:ground_truth_replacement}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textit{Graphviz} & \textit{Mermaid} & \textit{PlantUML} \\
\midrule
Claude3.5-Sonnet  & 7.16  & 7.56  & 3.07  \\
GPT-4o             & 3.88  & 6.14  & -1.02 \\
Qwen2.5-32B        & 4.50  & 6.34  & -3.27 \\
Llama3.1-70B      & 4.09  & 6.34  & 2.25  \\
Qwen2.5-14B        & 2.66  & 6.14  & 1.02  \\
Qwen2.5-72B        & 2.31  & 5.91  & -1.05 \\
Llama3.1-8B       & 5.53  & 2.25  & -2.46 \\
Qwen2.5-7B         & 4.30  & 5.80  & -0.55 \\
Mixtral-8x22B      & 1.84  & 1.64  & -1.02 \\
Phi3.5-MoE        & 1.23  & -0.20 & -2.04 \\
Phi3.5-Mini       & -1.23 & 0.50  & -2.56 \\
\bottomrule
\end{tabular}
\end{table}


==> table/information_content_evaluation.tex <==
\begin{table}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\setlength{\tabcolsep}{2pt} % Adjust column padding
\caption{Performance comparison of various LVLMs on the TextFlow pipeline, with evaluation conducted using GPT-4o as the reasoner.}
\label{tab:information_content_evluation}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{VQA} & \textbf{Graphviz} & \textbf{Mermaid} & \textbf{PlantUML} \\
\midrule
 Claude3.5-Sonnet & 76.61 & \underline{77.66} & \underline{\textbf{79.95}} & 66.43 \\
 GPT-4o & 65.69 & \underline{\textbf{80.10}} & \underline{77.81} & \underline{\textbf{66.83}} \\
 Qwen2-VL-72B & 64.14 & \underline{76.11} & \underline{75.26} & \underline{64.54} \\
 Qwen2-VL-7B & 53.42 & \underline{59.55} & \underline{60.35} & \underline{58.80} \\
 Llama3.2-90B & 43.09 & \underline{56.96} & \underline{64.09} & \underline{52.22} \\
 Llava-v1.6-110B & 42.69 & \underline{49.08} & \underline{45.94} & \underline{44.09} \\
 Llama3.2-11B & 8.33 & \underline{50.07} & \underline{50.47} & \underline{46.23} \\
\bottomrule
\end{tabular}
\end{table}


==> table/reasoner_evaluation.tex <==
\begin{table*}[ht!]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\caption{Total accuracy and detailed accuracy (by data source and tasks) of baseline VQA with GPT-4o and various LLMs using our Textflow pipeline. All text representations are extracted by GPT-4o. Rows with a grey background indicate closed-source models, while the remaining rows are open-source LLMs. Underscored values indicate results that outperform the baseline.}
\label{tab:reasoner_evalution}
\begin{tabular}{c|l|c|ccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Total}} & \multicolumn{3}{c|}{\textbf{Data Source}} & \multicolumn{4}{c}{\textbf{Tasks}} \\
\cmidrule(lr){4-10} & &  & \textbf{Code} & \textbf{Instruct} & \textbf{Wiki} & \textbf{$T_{1}$} & \textbf{$T_{2}$} & \textbf{$T_{3}$} & \textbf{$T_{4}$} \\
\midrule
\textbf{Image} & GPT-4o (VQA) & 65.69 & 78.23 & 69.37 & 59.96 & 73.83 & 68.16 & 69.80 & 58.91 \\

\midrule
\multirow{11}{*}{\begin{sideways}\textbf{Graphviz}\end{sideways}} 
& \cellcolor{lightgray}Claude3.5-Sonnet & \cellcolor{lightgray}\textbf{\underline{82.19}} & \cellcolor{lightgray}\textbf{91.48} & \cellcolor{lightgray}\textbf{84.27} & \cellcolor{lightgray}\textbf{78.32} & \cellcolor{lightgray}\textbf{90.12} & \cellcolor{lightgray}\textbf{81.84} & \cellcolor{lightgray}\textbf{76.07} & \cellcolor{lightgray}\textbf{81.11} \\
& \cellcolor{lightgray}GPT-4o & \cellcolor{lightgray}\underline{80.10} & \cellcolor{lightgray}87.07 & \cellcolor{lightgray}83.94 & \cellcolor{lightgray}75.92 & \cellcolor{lightgray}88.15 & \cellcolor{lightgray}81.34 & \cellcolor{lightgray}72.65 & \cellcolor{lightgray}78.75 \\
& Qwen2.5-32B & \underline{77.46} & 88.64 & 79.80 & 72.88 & 86.42 & 75.12 & 70.09 & 77.33 \\
& Llama3.1-70B & \underline{74.71} & 83.91 & 77.15 & 70.66 & 87.41 & 78.36 & 71.79 & 68.12 \\
& Qwen2.5-14B & \underline{74.51} & 87.38 & 77.48 & 69.10 & 81.98 & 72.39 & 68.09 & 74.62 \\
& Qwen2.5-72B & \underline{72.72} & 84.54 & 77.15 & 66.79 & 83.46 & 70.90 & 70.09 & 69.54 \\
& Mixtral-8x22B & \underline{67.03} & 76.03 & 69.54 & 63.01 & 86.17 & 73.13 & 66.38 & 55.25 \\
& Llama3.1-8B & 63.79 & 71.61 & 66.72 & 59.87 & 82.22 & 59.20 & 48.72 & 63.40 \\
& Qwen2.5-7B & 61.25 & 79.18 & 61.26 & 56.00 & 78.77 & 64.68 & 54.13 & 54.19 \\
& Phi3.5-MoE & 52.77 & 67.19 & 53.97 & 47.88 & 67.16 & 58.96 & 50.14 & 44.04 \\
& Phi3.5-Mini & 48.68 & 59.62 & 52.15 & 43.54 & 63.95 & 45.02 & 37.89 & 47.58 \\

\midrule
\multirow{11}{*} {\begin{sideways}\textbf{Mermaid}\end{sideways}} 
& \cellcolor{lightgray}Claude3.5-Sonnet & \cellcolor{lightgray}\underline{80.00} & \cellcolor{lightgray}90.85 & \cellcolor{lightgray}81.62 & \cellcolor{lightgray}75.92 & \cellcolor{lightgray}89.63 & \cellcolor{lightgray}80.85 & \cellcolor{lightgray}74.93 & \cellcolor{lightgray}77.10 \\ 
& \cellcolor{lightgray}GPT-4o & \cellcolor{lightgray}\underline{77.81} & \cellcolor{lightgray}88.33 & \cellcolor{lightgray}81.46 & \cellcolor{lightgray}72.69 & \cellcolor{lightgray}88.89 & \cellcolor{lightgray}79.10 & \cellcolor{lightgray}74.93 & \cellcolor{lightgray}73.08 \\
& Qwen2.5-32B & \underline{74.76} & 86.75 & 76.16 & 70.48 & 84.94 & 72.14 & 70.94 & 72.73 \\
& Llama3.1-70B & \underline{74.41} & 81.07 & 76.99 & 71.03 & 88.40 & 81.09 & 69.52 & 66.59 \\
& Qwen2.5-14B & \underline{73.37} & 85.17 & 74.01 & 69.56 & 85.93 & 72.89 & 72.08 & 68.12 \\
& Qwen2.5-72B & \underline{70.67} & 86.12 & 72.52 & 65.13 & 84.69 & 67.91 & 70.09 & 65.53 \\
& Llama3.1-8B & \underline{66.03} & 74.76 & 66.39 & 63.28 & 86.67 & 67.91 & 61.82 & 57.02 \\
& Mixtral-8x22B & 63.89 & 74.45 & 64.57 & 60.42 & 85.43 & 76.37 & 67.24 & 46.28 \\
& Qwen2.5-7B & 63.44 & 74.45 & 63.58 & 60.15 & 84.20 & 63.93 & 57.83 & 55.61 \\
& Phi3.5-MoE & 54.71 & 67.19 & 52.98 & 52.03 & 73.83 & 64.18 & 54.42 & 41.20 \\
& Phi3.5-Mini & 54.51 & 62.46 & 54.47 & 52.21 & 72.84 & 59.70 & 51.85 & 44.39 \\

\midrule
\multirow{11}{*}{\begin{sideways}\textbf{PlantUML}\end{sideways}} 
& \cellcolor{lightgray}Claude3.5-Sonnet & \cellcolor{lightgray}\underline{70.17} & \cellcolor{lightgray}78.55 & \cellcolor{lightgray}73.01 & \cellcolor{lightgray}66.14 & \cellcolor{lightgray}84.69 & \cellcolor{lightgray}79.10 & \cellcolor{lightgray}68.95 & \cellcolor{lightgray}59.50 \\
& \cellcolor{lightgray}GPT-4o & \cellcolor{lightgray}\underline{66.83} & \cellcolor{lightgray}76.03 & \cellcolor{lightgray}70.03 & \cellcolor{lightgray}62.36 & \cellcolor{lightgray}85.93 & \cellcolor{lightgray}73.63 & \cellcolor{lightgray}68.95 & \cellcolor{lightgray}53.60 \\
& Qwen2.5-32B & 64.59 & 74.13 & 67.05 & 60.42 & 82.47 & 73.13 & 68.95 & 50.18 \\
& Llama3.1-70B & 61.85 & 67.19 & 63.41 & 59.41 & 84.20 & 78.36 & 69.23 & 40.26 \\
& Qwen2.5-72B & 61.00 & 68.14 & 62.42 & 58.12 & 80.25 & 66.17 & 68.95 & 46.04 \\
& Qwen2.5-14B & 60.70 & 67.51 & 61.59 & 58.21 & 82.96 & 69.65 & 66.38 & 43.45 \\
& Mixtral-8x22B & 57.41 & 62.15 & 57.78 & 55.81 & 82.96 & 75.87 & 63.82 & 33.77 \\
& Llama3.1-8B & 53.57 & 58.99 & 55.63 & 50.83 & 83.95 & 69.65 & 56.13 & 30.34 \\
& Qwen2.5-7B & 52.92 & 60.88 & 53.81 & 50.09 & 82.22 & 61.44 & 56.70 & 33.29 \\
& Phi3.5-MoE & 51.47 & 57.41 & 50.33 & 50.37 & 76.79 & 66.42 & 55.27 & 30.70 \\
& Phi3.5-Mini & 45.14 & 52.05 & 45.03 & 43.17 & 71.85 & 57.71 & 45.87 & 26.09 \\
\bottomrule
\end{tabular}
\end{table*}


==> table/reverse_study.tex <==
\begin{table}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\setlength{\tabcolsep}{5pt} % Adjust column padding
\caption{Comparison of GPT-4o’s Performance on Top-Down (Normal) and Bottom-Up (Reversed) Flowchart Configurations, Showing Accuracy Differences.}
\label{tab:reverse_study}
\begin{tabular}{lccc}
\toprule
\textbf{Configuration} & \textbf{Top-Down} & \textbf{Bottom-UP} & \textbf{Difference} \\
\midrule
Graphviz & 80.10 & 74.86 & 5.24 \\
Mermaid  & 77.81 & 72.82 & 4.99 \\
PlantUML & 66.83 & 64.34 & 2.49 \\
VQA      & 65.69 & 59.25 & 6.44 \\
\bottomrule
\end{tabular}
\end{table}


==> table/textflow_vs_vqa.tex <==
% \begin{table*}[ht]
% \small
% \centering
% \setlength{\tabcolsep}{2.5pt} 
% \caption{Comparison of different LVLM performance on VQA and the TextFlow pipeline. Asterisks (*) indicate results using GPT-4o on the representations extracted by the corresponding LVLM, which can be used to evaluate the quality of extraction.}
% \label{tab:textflow_vs_vqa}
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Model} & \textbf{VQA} & \textbf{Graphviz} & \textbf{Mermaid} & \textbf{PlantUML} & \textbf{Graphviz*} & \textbf{Mermaid*} & \textbf{PlantUML*} \\
% \midrule
%  Claude3.5-Sonnet & \textbf{76.61} & \textbf{82.74} & \textbf{82.04} & \textbf{71.22} & 77.66 & \textbf{79.95} & 66.43 \\
%  GPT-4o & 65.69 & 80.10 & 77.81 & 66.83 & \textbf{80.10} & 77.81 & \textbf{66.83} \\
%  Qwen2-VL-72B & 64.14 & 64.64 & 62.19 & 57.91 & 76.11 & 75.26 & 64.54 \\
%  Qwen2-VL-7B & 53.42 & 48.43 & 49.93 & 46.18 & 59.55	& 60.35 & 58.80 \\
%  Llama3.2-90B & 43.09 & 53.97 & 62.29 & 49.93 & 56.96 & 64.09 & 52.22 \\
%  Llava-v1.6-110B & 42.69	& 43.09 & 43.24 & 39.50 & 49.08	& 45.94 & 44.09 \\
%  Llama3.2-11B & 8.33 & 39.80 & 41.40 & 34.21 & 50.07 & 50.47 & 46.23 \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\setlength{\tabcolsep}{2pt} % Adjust column padding
\caption{Comparison of different LVLM accuary on VQA and the TextFlow pipeline. The highest accuracy across models for each configurations is shown in bold. Underlined values indicate accuracy in the TextFlow pipeline that exceed the corresponding VQA pipeline for the same model.}
\label{tab:textflow_vs_vqa}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{VQA} & \textbf{Graphviz} & \textbf{Mermaid} & \textbf{PlantUML} \\
\midrule
 Claude3.5-Sonnet & \textbf{76.61} & \textbf{\underline{82.74}} & \textbf{\underline{82.04}} & \textbf{71.22} \\
 GPT-4o & 65.69 & \underline{80.10} & \underline{77.81} &  \underline{66.83} \\
 Qwen2-VL-72B & 64.14 & \underline{64.64} & 62.19 & 57.91 \\
 Qwen2-VL-7B & 53.42 & 48.43 & 49.93 & 46.18 \\
 Llama3.2-90B & 43.09 & \underline{53.97} & \underline{62.29} & \underline{49.93} \\
 Llava-v1.6-110B & 42.69 & \underline{43.09} & \underline{43.24} & 39.50 \\
 Llama3.2-11B & 8.33 & \underline{39.80} & \underline{41.40} & \underline{34.21} \\
\bottomrule
\end{tabular}
\end{table}



==> table/tool_evaluation.tex <==
\begin{table}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.2} % Increase row spacing for better readability
\setlength{\tabcolsep}{6pt} % Adjust column padding
\caption{GPT-4o' accuracy on Graphviz and Mermaid representations, comparing base and tool-assisted settings on extracted and ground truth (GT) representations. T4 represents topological tasks.}
\label{tab:tool_evaluation}
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{Overall} & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} \\
\midrule
\multicolumn{6}{c}{\textit{Graphviz}} \\
\midrule
Base & 80.10 & 88.15 & 81.34 & 72.65 & 78.75 \\
Tool & 80.79 & 84.94 & 80.60 & 70.37 & 83.23 \\
Base\textsuperscript{GT}  & 85.39 & 90.12 & 79.35 & 76.35 & 89.73 \\
Tool\textsuperscript{GT} & \textbf{88.23} & 86.91 & 79.35 & 72.08 & \textbf{99.76} \\
\midrule
\multicolumn{6}{c}{\textit{Mermaid}} \\
\midrule
Base & 77.81 & 88.89 & 79.10 & 74.93 & 73.08 \\
Tool & 78.89 & 86.91 & 79.35 & 69.52 & 78.87 \\
Base\textsuperscript{GT}  & 85.49 & 90.37 & 78.11 & 78.92 & 89.37 \\
Tool\textsuperscript{GT}  & \textbf{88.83} & 89.88 & 79.85 & 70.94 & \textbf{100.00} \\
\bottomrule
\end{tabular}
\end{table}

